Constraints on (2060) Chiron's size, shape, and surrounding material from the November 2018 and September 2019 stellar occultations

After the discovery of rings around the largest known Centaur object, (10199) Chariklo, we carried out observation campaigns of stellar occultations produced by the second-largest known Centaur object, (2060) Chiron, to better characterize its physical properties and presence of material on its surroundings. We predicted and successfully observed two stellar occultations by Chiron. These observations were used to constrain its size and shape by fitting elliptical limbs with equivalent surface radii in agreement with radiometric measurements. Constraints on the (2060) Chiron shape are reported for the first time. Assuming an equivalent radius of R$_{equiv}$ = 105$^{+6}_{-7}$ km, we obtained a semi-major axis of a = 126 $\pm$ 22 km. Considering Chiron's true rotational light curve amplitude and assuming it has a Jacobi equilibrium shape, we were able to derive a 3D shape with a semi-axis of a = 126 $\pm$ 22 km, b = 109 $\pm$ 19 km, and c = 68 $\pm$ 13 km, implying in a volume-equivalent radius of R$_{vol}$ = 98 $\pm$ 17 km, implying a density of 1119 $\pm$ 4 kg m$^{-3}$. We determined the physical properties of the 2011 secondary events around Chiron, which may then be directly compared with those of Chariklo rings, as the same method was used. Data obtained from SAAO in 2018 do not show unambiguous evidence of the proposed rings, mainly due to the large sampling time. Meanwhile, we discarded the possible presence of a permanent ring similar to (10199) Chariklo's C1R in optical depth and extension. Using the first multi-chord stellar occultation by (2060) Chiron and considering it to have a Jacobi equilibrium shape, we derived its 3D shape. New observations of a stellar occultation by (2060) Chiron are needed to further investigate the material's properties around Chiron, such as the occultation predicted for September 10, 2023.

==> references.tex <==
\begin{thebibliography}{}

    \bibitem[Almeida et al.(2009)]{Almeida09} Almeida,A.~J.~C., Peixinho, N., Correia, A.~C.~M.,\ 2009, \aap, 508, 2, 1021-1030.   

    \bibitem[Assafin et al.(2011)]{Assafin11} Assafin, M., Vieira Martins, R., Camargo, J.~I.~B., et al.\ 2011, Gaia follow-up network for the solar system objects : Gaia FUN-SSO workshop proceedings, 85-88.
 
    \bibitem[Alvarez-Candal et al.(2014)]{Alvarez-Candal14} Alvarez-Candal, A., Ortiz, J.~L., Morales, N., et al.\ 2014, \aap, 571, A48.   
   
    \bibitem[Barucci et al.(2012)]{Barucci12} Barucci, M.~A., Merlin, F., Perna, D., et al.\ 2012, \aap, 539, A152.

    \bibitem[Benedetti-Rossi et al.(2016)]{Benedetti-Rossi16} Benedetti-Rossi, G., Sicardy, B., Buie, M.~W., et al.\ 2016, \aj, 152, 156.
 
    \bibitem[Benedetti-Rossi et al.(2019)]{Benedetti-Rossi19} Benedetti-Rossi, G., Santos-Sanz,~P., Ortiz, J.~L., et al.\ 2019, \aj, 158, 159.
    
    \bibitem[B{\'e}rard et al.(2017)]{Berard17} B{\'e}rard, D., Sicardy, B., Camargo, J.~I.~B., et al.\ 2017, \aj, 154, 144.
 
    \bibitem[Braga-Ribas et al.(2013)]{BR13} Braga-Ribas, F., Sicardy, B., Ortiz, J.~L., et al.\ 2013, \apj, 773, 26. %doi:10.1088/0004-637X/773/1/26
 
    \bibitem[Braga-Ribas et al.(2014)]{Braga-Ribas14} Braga-Ribas, F., Sicardy, B., Ortiz, J.~L., et al.\ 2014, \nat, 508, 72.

    \bibitem[Bus et al.(1996)]{Bus96} Bus, S.~J., Buie, M.~W., Schleicher, D.~G., et al.\ 1996, \icarus, 123, 2, 478-490.
 
    \bibitem[Dias-Oliveira et al.(2017)]{Dias-Oliveira17} Dias-Oliveira, A., Sicardy, B., Ortiz, J.~L., et al.\ 2017, \aj, 154, 22.
    
    \bibitem[Desmars et al.(2015)]{Desmars15} Desmars, J., Camargo, J. I. B., Braga-Ribas, F., et al.\ 2015, \aap, 584, A96.
 
    \bibitem[Desmars et al.(2019)]{Desmars19} Desmars, J., Meza, E., Sicardy, B., et al.\ 2019, \aap, 625, A43.
 
    \bibitem[Duffard et al.(2014)]{Duffard14} Duffard, R., Pinilla-Alonso, N., Santos-Sanz, P., et al.\ 2014, \aap, 564, A92.
 
    \bibitem[Elliot et al.(1995)]{Elliot95} Elliot, J.~L., Olkin, C.~B., Dunham, E.~W., et al.\ 1995, \nat, 373, 46.

    \bibitem[Elliot et al.(2010)]{Elliot10} Elliot, J.~L., Person, M.~J., Zuluaga, C.~A., et al.\ 2010, \nat, 465, 897.
    
    \bibitem[Fornasier et al.(2013)]{Fornasier13} Fornasier, S., Lellouch, E., M{\"u}ller, T., et al.\ 2013, \aap, 555, A15.
 
    \bibitem[Gaia collaboration et al. (2016a)]{Gaia16} Gaia Collaboration, Prust, T., de Bruijne, J. H. J., Brown, A. G. A., et al. 2016(a), \aap, 595, A1.
 
    \bibitem[Gaia collaboration et al. (2016b)]{Gaia16_1}Gaia Collaboration; Brown, A. G. A.; Vallenari, A.; et al. 2016(b). \aap, 595, A2.
  
    \bibitem[Gaia collaboration et al. (2018)]{Gaia18}Gaia Collaboration; Brown, A. G. A.; Vallenari, A.; et al. 2018. \aap, 616, A1.
 
    \bibitem[Gladman et al.(2008)]{Gladman08} Gladman, B., Marsden, B.~G., \& Vanlaerhoven, C.\ 2008, The Solar System Beyond Neptune, 43.
    
    \bibitem[Lebofsky et al.(1984)]{Lebofsky84} Lebofsky, L.~A., Tholen, D.~J., Rieke, G.~H., et al. \icarus, 532–537.

    \bibitem[Leiva et al.(2017)]{Leiva17} Leiva, R., Sicardy, B., Camargo, J.~I.~B., et al.\ 2017, \aj, 154, 159.
 
    \bibitem[Lellouch et al.(2013)]{Lellouch13} Lellouch, E., Santos-Sanz, P., Lacerda, P., et al.\ 2013, \aap, 557, A60.

    \bibitem[Lellouch et al.(2017)]{Lellouch17} Lellouch, E., Moreno, R., M\"ueller, T., et al.\ 2017, \aap, 608, A45.

    \bibitem[Lim et al.(2010)]{Lim10} Lim, T.~L., Stansberry, J., M{\"u}ller, T.~G., et al.\ 2010, \aap, 518, L148.

    \bibitem[Leiva et al.(2017)]{Leiva17} Leiva, R., Sicardy, B., Camargo, J.~I.~B., et al.\ 2017, \aj, 154, 159.
 
    \bibitem[Lellouch et al.(2013)]{Lellouch13} Lellouch, E., Santos-Sanz, P., Lacerda, P., et al.\ 2013, \aap, 557, A60.

    \bibitem[Lellouch et al.(2017)]{Lellouch17} Lellouch, E., Moreno, R., M\"ueller, T., et al.\ 2017, \aap, 608, A45.

    \bibitem[Lim et al.(2010)]{Lim10} Lim, T.~L., Stansberry, J., M{\"u}ller, T.~G., et al.\ 2010, \aap, 518, L148.
 
    \bibitem[Mommert et al.(2012)]{MM12} Mommert, M., Harris, A.~W., Kiss, C., et al.\ 2012, \aap, 541, A93.
    
    \bibitem[Morgado et al.(2021)]{Morgado21} Morgado, B.~E., Sicardy, B., Braga-Ribas, F., et al.\ 2021, \aap, 652, A141.

    \bibitem[M\"ueller et al.(2019)]{Mueller19} M\"ueller,T., Lellouch, E., Fornasier, S.\ 2019, arXiv e-prints, 1905.07158.
 
    \bibitem[Nesvorn{\'y}, \& Morbidelli(2012)]{Nesvorny12} Nesvorn{\'y}, D., \& Morbidelli, A.\ 2012, \aj, 144, 117.

    \bibitem[Ortiz et al.(2012)]{Ortiz12} Ortiz, J.~L., Sicardy, B., Braga-Ribas, F., et al.\ 2012, \nat, 491, 566.
 
    \bibitem[Ortiz et al.(2015)]{Ortiz15} Ortiz, J.~L., Duffard, R., Pinilla-Alonso, N., et al.\ 2015, \aap, 576, A18.
 
    \bibitem[Ortiz et al.(2017)]{Ortiz17} Ortiz, J.~L., Santos-Sanz, P., Sicardy, B., et al.\ 2017, \nat, 550, 219.
 
    \bibitem[P{\'a}l et al.(2012)]{Pal12} P{\'a}l, A., Kiss, C., M{\"u}ller, T.~G., et al.\ 2012, \aap, 541, L6.
    
    \bibitem[Perryman, M. (2012)]{Perryman12}Perryman, Michael.\ 2012, European Physical Journal, v. 37, n. 5, p. 745-792. 
    
    \bibitem[Ruprecht et al. (2015)]{Ruprecht15} Ruprecht. J. ~D., Bosh, A. ~S., Person, M. ~J., et al.\ 2015, \icarus, 252, 271-276.
    
    \bibitem[Santos-Sanz et al.(2012)]{Santos-Sanz12} Santos-Sanz, P., Lellouch, E., Fornasier, S., et al.\ 2012, \aap, 541, A92.
 
    \bibitem[Stern et al.(2019)]{Stern19} Stern, S. A., Weaver, H. A., Spencer, J. R., et al.\ 2019, \textit{Science}, 364, 6441, aaw9771.
 
    \bibitem[Schindler et al.(2017)]{Schindler17} Schindler, K., Wolf, J., Bardecker, J., et al.\ 2017, \aap, 600, A12.
 
    \bibitem[Sicardy et al.(2011)]{Sicardy11} Sicardy, B., Ortiz, J.~L., Assafin, M., et al.\ 2011, \nat, 478, 493.
    
    \bibitem[Souami et al.(2020)]{Souami20} Souami, D., Braga-Ribas, F., Sicardy, B., et al.\ 2020, \aap, 643, A125. %doi:10.1051/0004-6361/202038526

    \bibitem[van Belle (1999)]{Vanbelle99} van Belle, G.~T.\ 1999, \pasp, 111, 1515.%doi:10.1086/316462

    \bibitem[Thirouin et al.(2010)]{Thirouin10} Thirouin, A., Ortiz, J.~L., Duffard, R., et al.\ 2010, \aap, 522, A93.
 
    \bibitem[Van Leeuwen, F. (1997)]{vanLeeuwen97} Van Leeuwen, Floor\ 1997, \textit{Space Science Reviews}, 81, p. 201-409.
 
    \bibitem[Vilenius et al.(2012)]{Vilenius12} Vilenius, E., Kiss, C., Mommert, M., et al.\ 2012, \aap, 541, A94.

    \bibitem[Vilenius et al.(2014)]{Vilenius14} Vilenius, E., Kiss, C., M\"ueller, T., et al.\ 2014, \aap, 564, A35.
 
    \bibitem[Zacharias et al.(2013)]{Zacharias13} Zacharias, N., Finch, C.~T., Girard, T.~M., et al.\ 2013, \aj, 145, 44.

\end{thebibliography}

